Zero-Shot Learning of Text Adventure Games with Sentence-Level Semantics

Reinforcement learning algorithms such as Q-learning have shown great promise in training models to learn the optimal action to take for a given system state; a goal in applications with an exploratory or adversarial nature such as task-oriented dialogues or games. However, models that do not have direct access to their state are harder to train; when the only state access is via the medium of language, this can be particularly pronounced. We introduce a new model amenable to deep Q-learning that incorporates a Siamese neural network architecture and a novel refactoring of the Q-value function in order to better represent system state given its approximation over a language channel. We evaluate the model in the context of zero-shot text-based adventure game learning. Extrinsically, our model reaches the baseline's convergence performance point needing only 15% of its iterations, reaches a convergence performance point 15% higher than the baseline's, and is able to play unseen, unrelated games with no fine-tuning. We probe our new model's representation space to determine that intrinsically, this is due to the appropriate clustering of different linguistic mediation into the same state.

==> ACL'20%20SNN-DRRN/tsne.tex <==
\begin{figure*}[ht]
  \centering
  \begin{subfigure}[b]{0.33\linewidth}
    \centering\includegraphics[width=140pt]{dqn-w-labels.pdf}
    \caption{DQN}
  \end{subfigure}%
  \begin{subfigure}[b]{0.33\linewidth}
    \centering\includegraphics[width=140pt]{dsqn-w-labels.pdf}
    \caption{DSQN}
  \end{subfigure}%
   \begin{subfigure}[b]{0.33\linewidth}
    \centering\includegraphics[width=140pt]{dsqn-q-fac-w-labels.pdf}
    \caption{DSQN + Q-factorization}
  \end{subfigure}
  \caption{t-SNE of language features learned by DQN, DSQN, and DSQN  with Q-factorization. There are 95 unique game states and 5,824 trajectories. Different colors indicate different unique game states. DSQN with Q-factorization clusters the game state nicely.}
  \label{fig:tsne}
\end{figure*}

